Scalarizing Functions in Bayesian Multiobjective Optimization

Scalarizing functions have been widely used to convert a multiobjective optimization problem into a single objective optimization problem. However, their use in solving (computationally) expensive multi- and many-objective optimization problems in Bayesian multiobjective optimization is scarce. Scalarizing functions can play a crucial role on the quality and number of evaluations required when doing the optimization. In this article, we study and review 15 different scalarizing functions in the framework of Bayesian multiobjective optimization and build Gaussian process models (as surrogates, metamodels or emulators) on them. We use expected improvement as infill criterion (or acquisition function) to update the models. In particular, we compare different scalarizing functions and analyze their performance on several benchmark problems with different number of objectives to be optimized. The review and experiments on different functions provide useful insights when using and selecting a scalarizing function when using a Bayesian multiobjective optimization method.

==> HV_DTLZ_Table.tex <==
\begin{table*} 
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|} 
\hline 
Problem & k& WS& EWC& WPO& WN& WPR& TCH& ATCH& MTCH \\ 
 \hline
 & 2& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 DTLZ1& 3& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 5& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 10& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\\hline
 & 2& 0.58 (0.01)& {\color{black}{\underline{0.53}}} (0.03)& {\color{black}\mymk{\textbf{0.64}}} (0.00)& 0.57 (0.01)& 0.57 (0.01)& {\color{black}{\textbf{0.63}}} (0.00)& {\color{black}{\textbf{0.63}}} (0.00)& {\color{black}{\textbf{0.63}}} (0.00)\\
 DTLZ2& 3& 0.74 (0.01)& {\color{black}{\underline{0.67}}} (0.03)& {\color{black}{\textbf{0.78}}} (0.00)& 0.73 (0.01)& 0.74 (0.01)& {\color{black}{\textbf{0.78}}} (0.00)& {\color{black}{\textbf{0.78}}} (0.00)& {\color{black}{\textbf{0.78}}} (0.00)\\
 & 5& 0.88 (0.01)& 0.74 (0.04)& 0.89 (0.01)& 0.88 (0.01)& 0.89 (0.01)& 0.87 (0.01)& 0.88 (0.01)& 0.88 (0.01)\\
 & 10& {\color{black}{\textbf{0.84}}} (0.03)& 0.73 (0.03)& {\color{black}{\textbf{0.87}}} (0.02)& {\color{black}{\textbf{0.85}}} (0.04)& 0.82 (0.03)& {\color{black}{\textbf{0.86}}} (0.03)& {\color{black}{\textbf{0.85}}} (0.03)& {\color{black}{\textbf{0.85}}} (0.02)\\\hline
 & 2& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 DTLZ3& 3& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 5& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 10& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\\hline
 & 2& {\color{black}{\textbf{0.54}}} (0.03)& 0.40 (0.08)& {\color{black}{\textbf{0.55}}} (0.01)& 0.45 (0.09)& {\color{black}{\underline{0.38}}} (0.07)& {\color{black}{\textbf{0.56}}} (0.01)& {\color{black}{\textbf{0.56}}} (0.00)& {\color{black}{\textbf{0.56}}} (0.00)\\
 DTLZ4& 3& 0.61 (0.07)& 0.50 (0.08)& {\color{black}{\textbf{0.70}}} (0.00)& {\color{black}{\underline{0.48}}} (0.06)& 0.51 (0.08)& {\color{black}{\textbf{0.65}}} (0.06)& {\color{black}{\textbf{0.65}}} (0.04)& {\color{black}{\textbf{0.67}}} (0.05)\\
 & 5& 0.71 (0.06)& 0.63 (0.09)& {\color{black}{\textbf{0.85}}} (0.01)& 0.71 (0.06)& 0.59 (0.09)& {\color{black}{\textbf{0.73}}} (0.06)& 0.69 (0.10)& 0.70 (0.10)\\
 & 10& {\color{black}{\textbf{0.89}}} (0.04)& 0.82 (0.05)& {\color{black}{\textbf{0.91}}} (0.03)& {\color{black}{\textbf{0.88}}} (0.04)& 0.78 (0.05)& {\color{black}{\textbf{0.90}}} (0.05)& {\color{black}{\textbf{0.90}}} (0.03)& {\color{black}{\textbf{0.90}}} (0.04)\\\hline
 & 2& 0.58 (0.01)& {\color{black}{\underline{0.53}}} (0.02)& {\color{black}\mymk{\textbf{0.63}}} (0.00)& 0.57 (0.01)& 0.57 (0.01)& {\color{black}{\textbf{0.63}}} (0.00)& {\color{black}{\textbf{0.63}}} (0.00)& {\color{black}{\textbf{0.63}}} (0.00)\\
 DTLZ5& 3& 0.47 (0.00)& 0.43 (0.03)& {\color{black}\mymk{\textbf{0.52}}} (0.01)& 0.47 (0.00)& 0.46 (0.01)& {\color{black}{\textbf{0.51}}} (0.00)& {\color{black}{\textbf{0.51}}} (0.00)& {\color{black}{\textbf{0.51}}} (0.01)\\
 & 5& 0.40 (0.01)& 0.34 (0.03)& {\color{black}{\textbf{0.43}}} (0.00)& 0.40 (0.01)& 0.40 (0.01)& 0.42 (0.01)& 0.42 (0.01)& 0.42 (0.00)\\
 & 10& 0.36 (0.01)& 0.31 (0.03)& {\color{black}{\textbf{0.39}}} (0.00)& 0.37 (0.00)& 0.37 (0.01)& 0.37 (0.00)& {\color{black}{\textbf{0.37}}} (0.00)& {\color{black}{\textbf{0.37}}} (0.01)\\\hline
 & 2& {\color{black}{\textbf{0.51}}} (0.06)& {\color{black}{\underline{0.00}}} (0.00)& {\color{black}{\textbf{0.48}}} (0.08)& {\color{black}{\textbf{0.53}}} (0.04)& 0.24 (0.19)& {\color{black}{\textbf{0.53}}} (0.03)& {\color{black}{\textbf{0.53}}} (0.07)& {\color{black}{\textbf{0.52}}} (0.07)\\
 DTLZ6& 3& {\color{black}{\textbf{0.32}}} (0.10)& {\color{black}{\underline{0.00}}} (0.00)& 0.15 (0.10)& 0.25 (0.13)& 0.09 (0.10)& {\color{black}{\textbf{0.34}}} (0.10)& {\color{black}{\textbf{0.30}}} (0.09)& {\color{black}{\textbf{0.35}}} (0.09)\\
 & 5& 0.05 (0.06)& {\color{black}{\underline{0.00}}} (0.00)& 0.01 (0.04)& 0.08 (0.09)& 0.01 (0.01)& 0.05 (0.08)& 0.05 (0.08)& 0.01 (0.04)\\
 & 10& {\color{black}{\underline{0.00}}} (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.01)& 0.00 (0.00)\\\hline
 & 2& 0.23 (0.01)& {\color{black}{\underline{0.00}}} (0.00)& 0.20 (0.03)& 0.26 (0.02)& 0.19 (0.03)& 0.23 (0.01)& 0.23 (0.02)& 0.23 (0.01)\\
 DTLZ7& 3& 0.21 (0.03)& {\color{black}{\underline{0.00}}} (0.00)& 0.18 (0.02)& 0.17 (0.01)& 0.17 (0.02)& 0.22 (0.01)& 0.21 (0.02)& 0.22 (0.01)\\
 & 5& {\color{black}{\textbf{0.15}}} (0.00)& {\color{black}{\underline{0.00}}} (0.00)& 0.04 (0.04)& {\color{black}{\textbf{0.15}}} (0.00)& 0.12 (0.02)& 0.15 (0.01)& {\color{black}{\textbf{0.15}}} (0.01)& 0.15 (0.01)\\
 & 10& {\color{black}{\textbf{0.05}}} (0.01)& {\color{black}{\underline{0.00}}} (0.00)& 0.00 (0.01)& {\color{black}\mymk{\textbf{0.08}}} (0.01)& 0.03 (0.01)& 0.03 (0.01)& 0.05 (0.01)& 0.04 (0.01)\\\hline
\end{tabular} 
\begin{tabular}{|l|l|c|c|c|c|c|c|c|} 
\hline 
Problem & k& PBI& IPBI& HypI& DomRank& MSD& QPBI& APD \\ 
 \hline
 & 2& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 DTLZ1& 3& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 5& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 10& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\\hline
 & 2& 0.61 (0.01)& {\color{black}{\textbf{0.62}}} (0.00)& 0.61 (0.01)& 0.61 (0.00)& 0.60 (0.02)& 0.61 (0.01)& {\color{black}{\textbf{0.63}}} (0.01)\\
 DTLZ2& 3& {\color{black}{\textbf{0.78}}} (0.00)& 0.68 (0.02)& {\color{black}\mymk{\textbf{0.79}}} (0.01)& 0.73 (0.02)& 0.77 (0.01)& {\color{black}{\textbf{0.77}}} (0.01)& {\color{black}{\textbf{0.79}}} (0.00)\\
 & 5& {\color{black}{\textbf{0.94}}} (0.00)& {\color{black}{\underline{0.65}}} (0.02)& 0.88 (0.02)& 0.78 (0.02)& 0.84 (0.07)& {\color{black}{\textbf{0.94}}} (0.00)& {\color{black}\mymk{\textbf{0.94}}} (0.00)\\
 & 10& {\color{black}{\textbf{0.84}}} (0.03)& {\color{black}{\underline{0.68}}} (0.01)& {\color{black}{\textbf{0.86}}} (0.06)& 0.77 (0.02)& {\color{black}{\textbf{0.84}}} (0.02)& {\color{black}{\textbf{0.86}}} (0.02)& {\color{black}\mymk{\textbf{0.88}}} (0.03)\\\hline
 & 2& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 DTLZ3& 3& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 5& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\
 & 10& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)\\\hline
 & 2& {\color{black}{\textbf{0.56}}} (0.01)& {\color{black}{\textbf{0.54}}} (0.02)& {\color{black}{\textbf{0.55}}} (0.02)& {\color{black}{\textbf{0.53}}} (0.02)& {\color{black}{\textbf{0.54}}} (0.04)& {\color{black}{\textbf{0.52}}} (0.06)& {\color{black}\mymk{\textbf{0.57}}} (0.02)\\
 DTLZ4& 3& {\color{black}{\textbf{0.71}}} (0.01)& 0.58 (0.11)& {\color{black}{\textbf{0.62}}} (0.10)& 0.58 (0.04)& {\color{black}{\textbf{0.69}}} (0.06)& {\color{black}{\textbf{0.71}}} (0.01)& {\color{black}\mymk{\textbf{0.72}}} (0.02)\\
 & 5& {\color{black}\mymk{\textbf{0.87}}} (0.02)& 0.56 (0.13)& {\color{black}{\underline{0.50}}} (0.13)& 0.72 (0.09)& 0.56 (0.17)& {\color{black}{\textbf{0.82}}} (0.04)& {\color{black}{\textbf{0.87}}} (0.01)\\
 & 10& {\color{black}\mymk{\textbf{0.94}}} (0.03)& 0.64 (0.05)& {\color{black}{\underline{0.60}}} (0.06)& 0.87 (0.04)& {\color{black}{\textbf{0.89}}} (0.03)& {\color{black}{\textbf{0.94}}} (0.02)& {\color{black}{\textbf{0.89}}} (0.06)\\\hline
 & 2& 0.61 (0.00)& {\color{black}{\textbf{0.62}}} (0.00)& 0.62 (0.01)& 0.61 (0.00)& 0.60 (0.02)& 0.61 (0.02)& {\color{black}{\textbf{0.63}}} (0.00)\\
 DTLZ5& 3& {\color{black}{\textbf{0.52}}} (0.00)& {\color{black}{\underline{0.42}}} (0.03)& {\color{black}{\textbf{0.50}}} (0.01)& 0.49 (0.01)& 0.50 (0.01)& {\color{black}{\textbf{0.51}}} (0.03)& {\color{black}{\textbf{0.52}}} (0.00)\\
 & 5& {\color{black}{\textbf{0.44}}} (0.01)& {\color{black}{\underline{0.31}}} (0.03)& 0.41 (0.01)& 0.41 (0.01)& 0.43 (0.01)& {\color{black}{\textbf{0.44}}} (0.00)& {\color{black}\mymk{\textbf{0.45}}} (0.00)\\
 & 10& {\color{black}{\textbf{0.38}}} (0.01)& {\color{black}{\underline{0.29}}} (0.03)& 0.31 (0.03)& 0.33 (0.02)& {\color{black}{\textbf{0.38}}} (0.01)& {\color{black}{\textbf{0.38}}} (0.00)& {\color{black}\mymk{\textbf{0.40}}} (0.00)\\\hline
 & 2& {\color{black}\mymk{\textbf{0.56}}} (0.01)& 0.01 (0.02)& 0.34 (0.22)& 0.34 (0.27)& {\color{black}{\textbf{0.49}}} (0.06)& 0.14 (0.10)& {\color{black}{\textbf{0.45}}} (0.10)\\
 DTLZ6& 3& {\color{black}\mymk{\textbf{0.42}}} (0.06)& 0.01 (0.01)& 0.02 (0.06)& 0.00 (0.00)& 0.22 (0.18)& 0.11 (0.08)& {\color{black}{\textbf{0.35}}} (0.07)\\
 & 5& {\color{black}\mymk{\textbf{0.33}}} (0.04)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.19 (0.07)\\
 & 10& {\color{black}\mymk{\textbf{0.17}}} (0.05)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.00 (0.00)& 0.03 (0.05)\\\hline
 & 2& 0.23 (0.01)& 0.17 (0.00)& {\color{black}\mymk{\textbf{0.31}}} (0.01)& 0.18 (0.04)& 0.24 (0.06)& 0.12 (0.02)& 0.25 (0.03)\\
 DTLZ7& 3& 0.17 (0.02)& 0.14 (0.02)& {\color{black}\mymk{\textbf{0.31}}} (0.04)& 0.14 (0.02)& 0.20 (0.05)& 0.11 (0.05)& 0.21 (0.04)\\
 & 5& 0.12 (0.03)& 0.00 (0.00)& {\color{black}\mymk{\textbf{0.19}}} (0.03)& 0.03 (0.03)& 0.11 (0.05)& 0.06 (0.02)& 0.13 (0.03)\\
 & 10& {\color{black}{\textbf{0.07}}} (0.02)& 0.00 (0.00)& 0.03 (0.04)& 0.01 (0.02)& 0.00 (0.00)& 0.01 (0.01)& 0.02 (0.03)\\\hline
\end{tabular} 
\caption{\label{tab:HV_DTLZ}Mean hypervolume values and standard deviation (in parentheses) for DTLZ problems. The values statistically similar to the best one are in bold, the best value is encircled the worst value is underlined}
\end{table*}

==> HV_WFG_Table.tex <==
\begin{table*} 
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|} 
\hline 
Problem & k& WS& EWC& WPO& WN& WPR& TCH& ATCH& MTCH \\ 
 \hline
 & 2& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\underline{0.09}}} (0.06)& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\textbf{0.22}}} (0.00)\\
 WFG1& 3& {\color{black}{\textbf{0.34}}} (0.00)& 0.20 (0.06)& {\color{black}{\textbf{0.34}}} (0.00)& {\color{black}{\textbf{0.34}}} (0.00)& {\color{black}{\textbf{0.33}}} (0.01)& {\color{black}{\textbf{0.34}}} (0.00)& {\color{black}{\textbf{0.34}}} (0.00)& {\color{black}\mymk{\textbf{0.34}}} (0.00)\\
 & 5& {\color{black}{\textbf{0.31}}} (0.00)& 0.23 (0.03)& {\color{black}{\textbf{0.31}}} (0.00)& {\color{black}\mymk{\textbf{0.31}}} (0.00)& {\color{black}{\textbf{0.31}}} (0.00)& {\color{black}{\textbf{0.31}}} (0.00)& {\color{black}{\textbf{0.31}}} (0.00)& {\color{black}{\textbf{0.31}}} (0.00)\\
 & 10& {\color{black}{\textbf{0.24}}} (0.00)& 0.16 (0.03)& {\color{black}{\textbf{0.23}}} (0.00)& {\color{black}\mymk{\textbf{0.24}}} (0.00)& {\color{black}{\textbf{0.23}}} (0.00)& {\color{black}{\textbf{0.24}}} (0.00)& {\color{black}{\textbf{0.24}}} (0.00)& {\color{black}{\textbf{0.23}}} (0.00)\\\hline
 & 2& {\color{black}{\textbf{0.49}}} (0.05)& {\color{black}{\underline{0.43}}} (0.03)& {\color{black}{\textbf{0.49}}} (0.03)& {\color{black}\mymk{\textbf{0.52}}} (0.05)& {\color{black}{\textbf{0.50}}} (0.04)& {\color{black}{\textbf{0.49}}} (0.03)& {\color{black}{\textbf{0.48}}} (0.03)& {\color{black}{\textbf{0.49}}} (0.03)\\
 WFG2& 3& {\color{black}{\textbf{0.66}}} (0.05)& 0.56 (0.05)& {\color{black}{\textbf{0.70}}} (0.04)& {\color{black}{\textbf{0.70}}} (0.04)& 0.63 (0.02)& 0.64 (0.04)& 0.64 (0.03)& 0.64 (0.03)\\
 & 5& {\color{black}{\textbf{0.77}}} (0.06)& 0.60 (0.06)& {\color{black}{\textbf{0.72}}} (0.05)& {\color{black}\mymk{\textbf{0.79}}} (0.05)& 0.68 (0.04)& {\color{black}{\textbf{0.73}}} (0.05)& {\color{black}{\textbf{0.72}}} (0.03)& {\color{black}{\textbf{0.72}}} (0.04)\\
 & 10& {\color{black}{\textbf{0.76}}} (0.07)& 0.58 (0.06)& {\color{black}{\textbf{0.70}}} (0.06)& {\color{black}\mymk{\textbf{0.80}}} (0.05)& 0.67 (0.06)& 0.68 (0.09)& 0.68 (0.08)& {\color{black}{\textbf{0.70}}} (0.06)\\\hline
 & 2& 0.49 (0.02)& {\color{black}{\underline{0.41}}} (0.02)& 0.51 (0.02)& 0.52 (0.01)& 0.46 (0.03)& 0.49 (0.01)& 0.49 (0.01)& 0.49 (0.01)\\
 WFG3& 3& 0.29 (0.02)& 0.26 (0.03)& 0.31 (0.01)& 0.29 (0.01)& {\color{black}{\underline{0.26}}} (0.01)& 0.27 (0.01)& 0.27 (0.01)& 0.27 (0.01)\\
 & 5& 0.13 (0.02)& {\color{black}{\underline{0.11}}} (0.02)& 0.14 (0.02)& 0.13 (0.02)& 0.13 (0.02)& 0.12 (0.02)& 0.12 (0.02)& 0.11 (0.02)\\
 & 10& 0.03 (0.01)& {\color{black}{\underline{0.02}}} (0.01)& {\color{black}{\textbf{0.04}}} (0.01)& {\color{black}{\textbf{0.04}}} (0.01)& 0.03 (0.01)& 0.03 (0.01)& 0.03 (0.01)& 0.03 (0.01)\\\hline
 & 2& {\color{black}\mymk{\textbf{0.35}}} (0.01)& {\color{black}{\underline{0.27}}} (0.02)& {\color{black}{\textbf{0.33}}} (0.01)& {\color{black}{\textbf{0.35}}} (0.02)& {\color{black}{\textbf{0.35}}} (0.01)& {\color{black}{\textbf{0.33}}} (0.01)& {\color{black}{\textbf{0.33}}} (0.01)& {\color{black}{\textbf{0.32}}} (0.02)\\
 WFG4& 3& {\color{black}{\textbf{0.46}}} (0.01)& 0.33 (0.03)& 0.40 (0.03)& {\color{black}\mymk{\textbf{0.48}}} (0.01)& 0.40 (0.01)& 0.41 (0.02)& 0.42 (0.02)& 0.42 (0.02)\\
 & 5& {\color{black}{\textbf{0.55}}} (0.04)& 0.33 (0.02)& 0.44 (0.03)& {\color{black}\mymk{\textbf{0.59}}} (0.03)& 0.42 (0.02)& 0.44 (0.03)& 0.45 (0.04)& 0.45 (0.03)\\
 & 10& 0.40 (0.04)& 0.28 (0.02)& 0.37 (0.04)& {\color{black}\mymk{\textbf{0.52}}} (0.02)& 0.33 (0.04)& 0.35 (0.04)& 0.36 (0.04)& 0.33 (0.03)\\\hline
 & 2& 0.29 (0.02)& {\color{black}{\underline{0.20}}} (0.01)& 0.27 (0.01)& 0.29 (0.02)& 0.28 (0.01)& 0.26 (0.01)& 0.26 (0.01)& 0.27 (0.01)\\
 WFG5& 3& {\color{black}{\textbf{0.34}}} (0.03)& {\color{black}{\underline{0.26}}} (0.01)& 0.33 (0.03)& {\color{black}{\textbf{0.36}}} (0.03)& {\color{black}{\textbf{0.34}}} (0.02)& 0.33 (0.02)& 0.32 (0.02)& 0.33 (0.02)\\
 & 5& 0.30 (0.02)& 0.26 (0.01)& 0.31 (0.02)& 0.31 (0.02)& 0.28 (0.02)& 0.31 (0.02)& 0.31 (0.02)& 0.31 (0.01)\\
 & 10& {\color{black}{\textbf{0.28}}} (0.02)& 0.24 (0.01)& 0.25 (0.02)& {\color{black}{\textbf{0.28}}} (0.01)& 0.26 (0.02)& {\color{black}{\textbf{0.28}}} (0.01)& {\color{black}{\textbf{0.28}}} (0.02)& {\color{black}{\textbf{0.27}}} (0.02)\\\hline
 & 2& 0.24 (0.03)& {\color{black}{\underline{0.21}}} (0.02)& 0.26 (0.02)& 0.27 (0.03)& 0.24 (0.03)& 0.23 (0.02)& 0.23 (0.02)& 0.23 (0.02)\\
 WFG6& 3& 0.30 (0.01)& 0.27 (0.02)& 0.33 (0.02)& 0.32 (0.03)& 0.30 (0.02)& 0.30 (0.01)& 0.31 (0.01)& 0.31 (0.01)\\
 & 5& 0.39 (0.02)& 0.28 (0.01)& 0.39 (0.01)& 0.36 (0.02)& 0.39 (0.02)& 0.40 (0.01)& 0.40 (0.01)& 0.40 (0.01)\\
 & 10& 0.29 (0.02)& 0.25 (0.01)& 0.28 (0.02)& 0.27 (0.02)& {\color{black}{\textbf{0.32}}} (0.02)& {\color{black}{\textbf{0.32}}} (0.03)& {\color{black}\mymk{\textbf{0.32}}} (0.02)& {\color{black}{\textbf{0.32}}} (0.02)\\\hline
 & 2& 0.28 (0.03)& 0.24 (0.01)& 0.31 (0.01)& 0.32 (0.02)& 0.25 (0.02)& 0.26 (0.01)& 0.26 (0.01)& 0.26 (0.01)\\
 WFG7& 3& 0.32 (0.02)& {\color{black}{\underline{0.30}}} (0.02)& {\color{black}{\textbf{0.42}}} (0.02)& 0.36 (0.04)& 0.32 (0.03)& 0.32 (0.02)& 0.33 (0.01)& 0.33 (0.01)\\
 & 5& 0.30 (0.03)& 0.29 (0.01)& 0.29 (0.01)& 0.31 (0.01)& 0.29 (0.02)& {\color{black}{\underline{0.28}}} (0.01)& 0.28 (0.01)& 0.28 (0.02)\\
 & 10& 0.27 (0.01)& 0.28 (0.01)& 0.28 (0.01)& 0.27 (0.02)& 0.27 (0.01)& 0.27 (0.01)& {\color{black}{\underline{0.26}}} (0.01)& 0.27 (0.01)\\\hline
 & 2& 0.17 (0.01)& 0.16 (0.01)& 0.17 (0.01)& {\color{black}{\underline{0.16}}} (0.01)& 0.17 (0.02)& 0.16 (0.01)& 0.16 (0.01)& 0.16 (0.01)\\
 WFG8& 3& 0.22 (0.02)& {\color{black}{\underline{0.21}}} (0.02)& {\color{black}{\textbf{0.25}}} (0.01)& 0.23 (0.03)& {\color{black}{\textbf{0.24}}} (0.02)& {\color{black}{\textbf{0.23}}} (0.01)& {\color{black}{\textbf{0.24}}} (0.01)& {\color{black}{\textbf{0.25}}} (0.01)\\
 & 5& 0.24 (0.01)& 0.23 (0.02)& 0.27 (0.01)& 0.24 (0.02)& 0.24 (0.01)& 0.24 (0.01)& 0.23 (0.01)& 0.24 (0.01)\\
 & 10& 0.23 (0.01)& 0.24 (0.01)& 0.24 (0.01)& 0.23 (0.01)& 0.24 (0.01)& {\color{black}{\textbf{0.25}}} (0.01)& 0.24 (0.01)& 0.24 (0.01)\\\hline
 & 2& 0.33 (0.02)& {\color{black}{\underline{0.24}}} (0.03)& 0.30 (0.02)& 0.30 (0.04)& 0.29 (0.04)& 0.30 (0.03)& 0.29 (0.02)& 0.29 (0.02)\\
 WFG9& 3& {\color{black}{\textbf{0.38}}} (0.05)& 0.27 (0.02)& 0.36 (0.02)& 0.35 (0.03)& 0.33 (0.03)& 0.36 (0.04)& 0.36 (0.03)& 0.37 (0.03)\\
 & 5& 0.30 (0.03)& 0.27 (0.02)& 0.29 (0.02)& 0.28 (0.04)& 0.28 (0.02)& 0.31 (0.03)& 0.30 (0.02)& 0.30 (0.02)\\
 & 10& 0.28 (0.02)& 0.27 (0.01)& 0.27 (0.01)& 0.29 (0.02)& 0.26 (0.01)& 0.28 (0.01)& 0.28 (0.01)& 0.27 (0.01)\\\hline
\end{tabular} 
\begin{tabular}{|l|l|c|c|c|c|c|c|c|} 
\hline 
Problem & k& PBI& IPBI& HypI& DomRank& MSD& QPBI& APD \\ 
 \hline
 & 2& {\color{black}\mymk{\textbf{0.23}}} (0.01)& {\color{black}{\textbf{0.22}}} (0.00)& {\color{black}{\textbf{0.19}}} (0.07)& {\color{black}{\textbf{0.21}}} (0.01)& {\color{black}{\textbf{0.20}}} (0.02)& 0.15 (0.03)& {\color{black}{\textbf{0.19}}} (0.02)\\
 WFG1& 3& {\color{black}{\textbf{0.31}}} (0.02)& 0.28 (0.04)& {\color{black}{\underline{0.15}}} (0.13)& {\color{black}{\textbf{0.32}}} (0.01)& {\color{black}{\textbf{0.34}}} (0.01)& 0.25 (0.02)& {\color{black}{\textbf{0.31}}} (0.02)\\
 & 5& {\color{black}{\textbf{0.27}}} (0.04)& 0.26 (0.03)& {\color{black}{\underline{0.14}}} (0.08)& {\color{black}{\textbf{0.28}}} (0.01)& {\color{black}{\textbf{0.30}}} (0.03)& 0.21 (0.07)& {\color{black}{\textbf{0.28}}} (0.02)\\
 & 10& 0.18 (0.03)& {\color{black}{\textbf{0.21}}} (0.02)& 0.11 (0.06)& {\color{black}{\textbf{0.22}}} (0.02)& 0.18 (0.03)& {\color{black}{\underline{0.10}}} (0.06)& 0.15 (0.04)\\\hline
 & 2& {\color{black}{\textbf{0.52}}} (0.04)& 0.46 (0.03)& {\color{black}{\textbf{0.50}}} (0.04)& {\color{black}{\textbf{0.48}}} (0.03)& {\color{black}{\textbf{0.50}}} (0.03)& {\color{black}{\textbf{0.47}}} (0.03)& {\color{black}{\textbf{0.47}}} (0.03)\\
 WFG2& 3& 0.63 (0.05)& 0.60 (0.04)& {\color{black}{\underline{0.53}}} (0.03)& 0.64 (0.05)& {\color{black}\mymk{\textbf{0.73}}} (0.05)& 0.60 (0.06)& 0.64 (0.06)\\
 & 5& {\color{black}{\textbf{0.73}}} (0.11)& {\color{black}{\textbf{0.70}}} (0.06)& {\color{black}{\underline{0.59}}} (0.04)& {\color{black}{\textbf{0.71}}} (0.05)& {\color{black}{\textbf{0.73}}} (0.10)& 0.67 (0.06)& {\color{black}{\textbf{0.73}}} (0.10)\\
 & 10& {\color{black}{\textbf{0.77}}} (0.09)& 0.65 (0.06)& {\color{black}{\underline{0.57}}} (0.05)& 0.60 (0.03)& 0.64 (0.06)& 0.66 (0.07)& 0.63 (0.06)\\\hline
 & 2& 0.47 (0.01)& 0.42 (0.02)& {\color{black}\mymk{\textbf{0.56}}} (0.02)& 0.45 (0.02)& 0.52 (0.01)& 0.48 (0.01)& 0.53 (0.02)\\
 WFG3& 3& 0.32 (0.02)& 0.26 (0.02)& {\color{black}\mymk{\textbf{0.36}}} (0.03)& 0.28 (0.01)& 0.31 (0.02)& 0.33 (0.02)& 0.33 (0.03)\\
 & 5& {\color{black}\mymk{\textbf{0.21}}} (0.02)& 0.14 (0.02)& 0.16 (0.04)& 0.12 (0.02)& {\color{black}{\textbf{0.19}}} (0.03)& {\color{black}{\textbf{0.19}}} (0.02)& {\color{black}{\textbf{0.21}}} (0.02)\\
 & 10& {\color{black}\mymk{\textbf{0.06}}} (0.01)& 0.03 (0.01)& 0.02 (0.01)& 0.02 (0.01)& 0.02 (0.01)& {\color{black}{\textbf{0.05}}} (0.01)& {\color{black}{\textbf{0.04}}} (0.02)\\\hline
 & 2& {\color{black}{\textbf{0.34}}} (0.02)& 0.29 (0.03)& {\color{black}{\textbf{0.34}}} (0.03)& 0.28 (0.01)& 0.32 (0.03)& 0.29 (0.02)& 0.29 (0.02)\\
 WFG4& 3& {\color{black}{\textbf{0.46}}} (0.03)& 0.36 (0.03)& 0.40 (0.07)& 0.35 (0.03)& 0.38 (0.04)& {\color{black}{\underline{0.33}}} (0.05)& {\color{black}{\textbf{0.44}}} (0.04)\\
 & 5& {\color{black}{\textbf{0.59}}} (0.03)& 0.37 (0.04)& {\color{black}{\underline{0.31}}} (0.04)& 0.32 (0.02)& 0.35 (0.03)& 0.32 (0.02)& 0.48 (0.06)\\
 & 10& 0.39 (0.02)& 0.35 (0.02)& {\color{black}{\underline{0.25}}} (0.01)& 0.25 (0.01)& 0.26 (0.01)& 0.42 (0.02)& 0.36 (0.01)\\\hline
 & 2& 0.28 (0.01)& 0.22 (0.02)& {\color{black}\mymk{\textbf{0.35}}} (0.02)& {\color{black}{\textbf{0.33}}} (0.02)& 0.30 (0.01)& 0.23 (0.02)& 0.24 (0.03)\\
 WFG5& 3& {\color{black}{\textbf{0.35}}} (0.02)& 0.28 (0.02)& {\color{black}{\textbf{0.36}}} (0.06)& 0.34 (0.04)& {\color{black}\mymk{\textbf{0.38}}} (0.03)& 0.30 (0.03)& {\color{black}{\textbf{0.35}}} (0.03)\\
 & 5& {\color{black}\mymk{\textbf{0.38}}} (0.02)& 0.27 (0.01)& {\color{black}{\underline{0.25}}} (0.02)& 0.29 (0.02)& 0.30 (0.02)& 0.28 (0.01)& 0.34 (0.02)\\
 & 10& {\color{black}\mymk{\textbf{0.30}}} (0.02)& 0.24 (0.01)& {\color{black}{\underline{0.23}}} (0.01)& 0.23 (0.01)& 0.24 (0.01)& {\color{black}{\textbf{0.27}}} (0.02)& 0.27 (0.01)\\\hline
 & 2& {\color{black}{\textbf{0.31}}} (0.01)& 0.24 (0.02)& {\color{black}\mymk{\textbf{0.33}}} (0.03)& 0.22 (0.02)& {\color{black}{\textbf{0.30}}} (0.03)& 0.27 (0.03)& 0.26 (0.02)\\
 WFG6& 3& {\color{black}{\textbf{0.41}}} (0.02)& 0.31 (0.02)& 0.36 (0.08)& {\color{black}{\underline{0.26}}} (0.02)& 0.36 (0.02)& 0.35 (0.05)& {\color{black}\mymk{\textbf{0.42}}} (0.03)\\
 & 5& {\color{black}\mymk{\textbf{0.50}}} (0.04)& 0.31 (0.01)& {\color{black}{\underline{0.27}}} (0.04)& 0.28 (0.02)& 0.29 (0.02)& 0.37 (0.06)& 0.44 (0.03)\\
 & 10& {\color{black}{\textbf{0.31}}} (0.03)& 0.26 (0.01)& {\color{black}{\underline{0.23}}} (0.01)& 0.23 (0.01)& 0.25 (0.01)& 0.29 (0.02)& 0.26 (0.01)\\\hline
 & 2& 0.29 (0.01)& {\color{black}{\underline{0.24}}} (0.01)& {\color{black}\mymk{\textbf{0.37}}} (0.02)& 0.29 (0.02)& {\color{black}{\textbf{0.35}}} (0.02)& 0.28 (0.01)& 0.30 (0.02)\\
 WFG7& 3& 0.39 (0.02)& 0.31 (0.02)& {\color{black}\mymk{\textbf{0.45}}} (0.03)& 0.37 (0.01)& 0.35 (0.03)& 0.38 (0.03)& 0.39 (0.02)\\
 & 5& {\color{black}\mymk{\textbf{0.44}}} (0.03)& 0.32 (0.02)& 0.37 (0.04)& 0.34 (0.01)& 0.32 (0.01)& 0.33 (0.05)& {\color{black}{\textbf{0.44}}} (0.03)\\
 & 10& 0.29 (0.02)& {\color{black}\mymk{\textbf{0.33}}} (0.01)& 0.29 (0.02)& 0.30 (0.01)& 0.30 (0.02)& 0.29 (0.02)& 0.30 (0.02)\\\hline
 & 2& 0.16 (0.01)& 0.17 (0.01)& {\color{black}\mymk{\textbf{0.21}}} (0.01)& 0.18 (0.01)& 0.17 (0.01)& 0.16 (0.01)& 0.17 (0.01)\\
 WFG8& 3& {\color{black}{\textbf{0.26}}} (0.01)& {\color{black}{\textbf{0.24}}} (0.02)& 0.23 (0.04)& {\color{black}{\textbf{0.23}}} (0.01)& {\color{black}{\textbf{0.24}}} (0.02)& {\color{black}{\textbf{0.25}}} (0.02)& {\color{black}\mymk{\textbf{0.26}}} (0.02)\\
 & 5& {\color{black}\mymk{\textbf{0.31}}} (0.03)& 0.26 (0.02)& {\color{black}{\underline{0.22}}} (0.03)& 0.24 (0.02)& 0.23 (0.01)& 0.25 (0.02)& 0.27 (0.02)\\
 & 10& 0.24 (0.01)& {\color{black}\mymk{\textbf{0.26}}} (0.02)& {\color{black}{\underline{0.23}}} (0.01)& 0.24 (0.01)& 0.23 (0.01)& 0.24 (0.01)& {\color{black}{\textbf{0.25}}} (0.01)\\\hline
 & 2& {\color{black}{\textbf{0.34}}} (0.02)& 0.25 (0.02)& {\color{black}\mymk{\textbf{0.38}}} (0.02)& 0.25 (0.02)& 0.29 (0.05)& 0.26 (0.04)& 0.27 (0.03)\\
 WFG9& 3& {\color{black}\mymk{\textbf{0.43}}} (0.04)& {\color{black}{\underline{0.26}}} (0.02)& 0.34 (0.09)& 0.35 (0.04)& {\color{black}{\textbf{0.39}}} (0.04)& 0.29 (0.03)& {\color{black}{\textbf{0.38}}} (0.04)\\
 & 5& {\color{black}\mymk{\textbf{0.44}}} (0.01)& {\color{black}{\underline{0.26}}} (0.01)& 0.28 (0.06)& 0.30 (0.02)& 0.34 (0.03)& 0.30 (0.03)& 0.37 (0.03)\\
 & 10& {\color{black}\mymk{\textbf{0.32}}} (0.02)& 0.27 (0.02)& {\color{black}{\underline{0.26}}} (0.01)& 0.27 (0.01)& 0.27 (0.01)& {\color{black}{\textbf{0.30}}} (0.02)& 0.28 (0.01)\\\hline
\end{tabular} 
\caption{\label{tab:HV_WFG}Mean hypervolume values and standard deviation (in parentheses) for DTLZ problems. The values statistically similar to the best one are in bold, the best value is encircled the worst value is underlined}
\end{table*}

==> IGD_WFG_Table.tex <==
\begin{table*} 
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|} 
\hline 
Problem & k& WS& EWC& WPO& WN& WPR& TCH& ATCH& MTCH \\ 
 \hline
 & 2& {\color{black}{\textbf{1.31}}} (0.00)& {\color{black}{\underline{1.68}}} (0.30)& {\color{black}{\textbf{1.30}}} (0.01)& {\color{black}{\textbf{1.31}}} (0.01)& {\color{black}{\textbf{1.31}}} (0.01)& {\color{black}{\textbf{1.31}}} (0.00)& {\color{black}{\textbf{1.30}}} (0.01)& {\color{black}{\textbf{1.31}}} (0.00)\\
 WFG1& 3& {\color{black}{\textbf{1.55}}} (0.01)& 1.82 (0.18)& {\color{black}\mymk{\textbf{1.55}}} (0.01)& {\color{black}{\textbf{1.55}}} (0.01)& {\color{black}{\textbf{1.56}}} (0.01)& {\color{black}{\textbf{1.55}}} (0.01)& {\color{black}{\textbf{1.55}}} (0.01)& {\color{black}{\textbf{1.55}}} (0.01)\\
 & 5& {\color{black}{\textbf{2.05}}} (0.01)& 2.36 (0.09)& {\color{black}\mymk{\textbf{2.04}}} (0.02)& {\color{black}{\textbf{2.05}}} (0.01)& {\color{black}{\textbf{2.07}}} (0.01)& {\color{black}{\textbf{2.04}}} (0.02)& {\color{black}{\textbf{2.05}}} (0.01)& {\color{black}{\textbf{2.05}}} (0.01)\\
 & 10& {\color{black}{\textbf{3.12}}} (0.03)& 3.58 (0.22)& {\color{black}{\textbf{3.13}}} (0.04)& {\color{black}\mymk{\textbf{3.10}}} (0.03)& {\color{black}{\textbf{3.12}}} (0.04)& {\color{black}{\textbf{3.11}}} (0.04)& {\color{black}{\textbf{3.10}}} (0.04)& {\color{black}{\textbf{3.11}}} (0.03)\\\hline
 & 2& {\color{black}{\textbf{0.38}}} (0.10)& {\color{black}{\underline{0.46}}} (0.07)& {\color{black}{\textbf{0.37}}} (0.07)& {\color{black}\mymk{\textbf{0.29}}} (0.07)& {\color{black}{\textbf{0.34}}} (0.06)& {\color{black}{\textbf{0.37}}} (0.07)& {\color{black}{\textbf{0.39}}} (0.06)& {\color{black}{\textbf{0.38}}} (0.06)\\
 WFG2& 3& 0.71 (0.09)& 0.75 (0.07)& 0.67 (0.05)& 0.68 (0.08)& 0.74 (0.06)& 0.72 (0.08)& 0.70 (0.08)& 0.71 (0.08)\\
 & 5& {\color{black}{\textbf{1.26}}} (0.20)& 1.74 (0.25)& {\color{black}{\textbf{1.30}}} (0.17)& {\color{black}{\textbf{1.25}}} (0.22)& {\color{black}{\textbf{1.46}}} (0.09)& {\color{black}{\textbf{1.28}}} (0.23)& {\color{black}{\textbf{1.26}}} (0.13)& {\color{black}\mymk{\textbf{1.22}}} (0.19)\\
 & 10& {\color{black}{\textbf{3.67}}} (0.34)& 4.23 (0.61)& {\color{black}{\textbf{3.86}}} (0.44)& {\color{black}\mymk{\textbf{3.34}}} (0.64)& {\color{black}{\textbf{3.81}}} (0.41)& {\color{black}{\textbf{4.04}}} (0.50)& {\color{black}{\textbf{3.85}}} (0.46)& {\color{black}{\textbf{3.96}}} (0.32)\\\hline
 & 2& 0.31 (0.05)& {\color{black}{\underline{0.49}}} (0.06)& 0.26 (0.03)& 0.25 (0.02)& 0.37 (0.05)& 0.32 (0.02)& 0.31 (0.02)& 0.32 (0.03)\\
 WFG3& 3& 0.49 (0.04)& 0.54 (0.06)& 0.38 (0.04)& 0.48 (0.02)& 0.55 (0.03)& 0.52 (0.03)& 0.52 (0.03)& 0.52 (0.04)\\
 & 5& 0.70 (0.04)& {\color{black}{\underline{0.76}}} (0.05)& 0.64 (0.05)& 0.68 (0.05)& 0.71 (0.05)& 0.71 (0.04)& 0.70 (0.04)& 0.71 (0.05)\\
 & 10& 1.04 (0.08)& {\color{black}{\underline{1.15}}} (0.08)& {\color{black}{\textbf{0.87}}} (0.09)& 1.03 (0.11)& 1.06 (0.12)& 1.07 (0.10)& 1.06 (0.11)& 1.06 (0.09)\\\hline
 & 2& {\color{black}{\textbf{0.21}}} (0.02)& {\color{black}{\underline{0.40}}} (0.09)& {\color{black}{\textbf{0.26}}} (0.05)& {\color{black}{\textbf{0.21}}} (0.03)& {\color{black}{\textbf{0.21}}} (0.03)& {\color{black}{\textbf{0.26}}} (0.04)& {\color{black}{\textbf{0.25}}} (0.06)& {\color{black}{\textbf{0.24}}} (0.04)\\
 WFG4& 3& {\color{black}{\textbf{0.56}}} (0.05)& 0.81 (0.16)& {\color{black}{\textbf{0.62}}} (0.05)& {\color{black}{\textbf{0.48}}} (0.04)& {\color{black}{\textbf{0.63}}} (0.06)& {\color{black}{\textbf{0.58}}} (0.08)& {\color{black}{\textbf{0.62}}} (0.06)& {\color{black}{\textbf{0.61}}} (0.04)\\
 & 5& {\color{black}{\textbf{1.64}}} (0.22)& 2.45 (0.27)& {\color{black}{\textbf{1.69}}} (0.13)& {\color{black}\mymk{\textbf{1.51}}} (0.14)& {\color{black}{\textbf{1.69}}} (0.07)& {\color{black}{\textbf{1.78}}} (0.13)& {\color{black}{\textbf{1.81}}} (0.10)& {\color{black}{\textbf{1.82}}} (0.24)\\
 & 10& 7.32 (0.50)& 10.43 (0.96)& 7.60 (0.29)& {\color{black}\mymk{\textbf{6.50}}} (0.29)& {\color{black}{\textbf{7.08}}} (0.45)& 7.82 (0.47)& 7.68 (0.40)& 7.97 (0.38)\\\hline
 & 2& {\color{black}{\textbf{0.28}}} (0.04)& {\color{black}{\underline{0.64}}} (0.05)& 0.38 (0.04)& {\color{black}{\textbf{0.29}}} (0.05)& 0.37 (0.04)& 0.40 (0.05)& 0.39 (0.05)& 0.40 (0.06)\\
 WFG5& 3& {\color{black}{\textbf{0.72}}} (0.09)& {\color{black}{\underline{0.93}}} (0.06)& 0.78 (0.11)& {\color{black}{\textbf{0.71}}} (0.09)& 0.80 (0.09)& 0.76 (0.07)& 0.76 (0.05)& 0.75 (0.06)\\
 & 5& 2.33 (0.12)& 2.39 (0.14)& 2.25 (0.11)& 2.36 (0.13)& 2.48 (0.18)& 2.29 (0.19)& 2.32 (0.20)& 2.34 (0.16)\\
 & 10& 9.27 (0.29)& 9.13 (0.39)& 9.07 (0.33)& 9.26 (0.27)& 9.22 (0.23)& 9.15 (0.32)& 9.10 (0.36)& 9.21 (0.28)\\\hline
 & 2& 0.40 (0.06)& {\color{black}{\underline{0.57}}} (0.08)& 0.39 (0.05)& 0.35 (0.06)& 0.41 (0.04)& 0.42 (0.03)& 0.42 (0.04)& 0.44 (0.04)\\
 WFG6& 3& 0.69 (0.02)& 0.88 (0.08)& 0.69 (0.03)& 0.71 (0.03)& 0.73 (0.04)& 0.69 (0.02)& 0.68 (0.02)& 0.69 (0.02)\\
 & 5& 1.65 (0.09)& 2.07 (0.09)& 1.63 (0.04)& 1.77 (0.08)& 1.67 (0.07)& {\color{black}{\textbf{1.58}}} (0.04)& {\color{black}{\textbf{1.57}}} (0.05)& {\color{black}{\textbf{1.57}}} (0.04)\\
 & 10& 8.14 (0.50)& 8.71 (0.31)& 8.52 (0.24)& 8.62 (0.31)& {\color{black}{\textbf{7.62}}} (0.39)& {\color{black}\mymk{\textbf{7.43}}} (0.48)& {\color{black}{\textbf{7.58}}} (0.43)& {\color{black}{\textbf{7.61}}} (0.40)\\\hline
 & 2& 0.42 (0.06)& {\color{black}{\underline{0.50}}} (0.06)& 0.27 (0.03)& 0.37 (0.06)& 0.43 (0.03)& 0.38 (0.01)& 0.38 (0.02)& 0.37 (0.02)\\
 WFG7& 3& 0.79 (0.03)& {\color{black}{\underline{0.90}}} (0.09)& 0.73 (0.04)& 0.77 (0.04)& 0.78 (0.02)& 0.79 (0.04)& 0.78 (0.05)& 0.77 (0.03)\\
 & 5& 2.18 (0.16)& {\color{black}{\underline{2.58}}} (0.16)& 2.20 (0.11)& 2.31 (0.24)& 2.25 (0.10)& 2.20 (0.12)& 2.15 (0.07)& 2.21 (0.12)\\
 & 10& 10.09 (0.35)& {\color{black}{\underline{10.17}}} (0.30)& {\color{black}{\textbf{9.75}}} (0.28)& 10.16 (0.42)& 10.10 (0.43)& {\color{black}{\textbf{9.57}}} (0.39)& {\color{black}{\textbf{9.59}}} (0.34)& {\color{black}{\textbf{9.83}}} (0.49)\\\hline
 & 2& {\color{black}{\textbf{0.68}}} (0.05)& {\color{black}{\underline{0.84}}} (0.10)& {\color{black}{\textbf{0.71}}} (0.05)& {\color{black}{\textbf{0.72}}} (0.06)& {\color{black}\mymk{\textbf{0.65}}} (0.04)& {\color{black}{\textbf{0.70}}} (0.03)& {\color{black}{\textbf{0.67}}} (0.03)& {\color{black}{\textbf{0.69}}} (0.03)\\
 WFG8& 3& {\color{black}{\textbf{0.99}}} (0.02)& 1.13 (0.10)& {\color{black}{\textbf{0.92}}} (0.03)& {\color{black}{\textbf{0.99}}} (0.03)& {\color{black}{\textbf{0.97}}} (0.02)& {\color{black}{\textbf{0.97}}} (0.02)& {\color{black}{\textbf{0.97}}} (0.02)& {\color{black}{\textbf{0.96}}} (0.02)\\
 & 5& 2.35 (0.13)& 2.78 (0.19)& 2.24 (0.12)& 2.51 (0.16)& 2.23 (0.09)& 2.27 (0.10)& 2.25 (0.11)& 2.28 (0.15)\\
 & 10& 9.80 (0.37)& 10.07 (0.25)& 9.49 (0.52)& 9.95 (0.32)& 9.75 (0.49)& 9.58 (0.39)& 9.51 (0.43)& 9.55 (0.52)\\\hline
 & 2& {\color{black}{\textbf{0.26}}} (0.07)& {\color{black}{\underline{0.49}}} (0.08)& 0.35 (0.07)& 0.29 (0.11)& 0.33 (0.12)& 0.34 (0.10)& 0.35 (0.07)& 0.36 (0.07)\\
 WFG9& 3& {\color{black}{\textbf{0.62}}} (0.10)& 0.91 (0.06)& 0.70 (0.07)& 0.70 (0.08)& 0.79 (0.06)& 0.68 (0.11)& 0.67 (0.07)& 0.66 (0.07)\\
 & 5& 2.35 (0.12)& 2.35 (0.15)& 2.33 (0.16)& {\color{black}{\underline{2.48}}} (0.23)& 2.42 (0.14)& 2.24 (0.17)& 2.33 (0.17)& 2.29 (0.12)\\
 & 10& {\color{black}{\textbf{9.26}}} (0.25)& {\color{black}\mymk{\textbf{9.13}}} (0.34)& {\color{black}{\textbf{9.20}}} (0.22)& {\color{black}{\textbf{9.22}}} (0.19)& {\color{black}{\textbf{9.22}}} (0.30)& {\color{black}{\textbf{9.19}}} (0.26)& {\color{black}{\textbf{9.22}}} (0.21)& {\color{black}{\textbf{9.23}}} (0.25)\\\hline
\end{tabular} 
\begin{tabular}{|l|l|c|c|c|c|c|c|c|} 
\hline 
Problem & k& PBI& IPBI& HypI& DomRank& MSD& QPBI& APD \\ 
 \hline
 & 2& {\color{black}\mymk{\textbf{1.29}}} (0.03)& {\color{black}{\textbf{1.31}}} (0.01)& {\color{black}{\textbf{1.39}}} (0.32)& {\color{black}{\textbf{1.29}}} (0.02)& {\color{black}{\textbf{1.33}}} (0.04)& {\color{black}{\textbf{1.42}}} (0.08)& {\color{black}{\textbf{1.34}}} (0.03)\\
 WFG1& 3& {\color{black}{\textbf{1.57}}} (0.03)& {\color{black}{\textbf{1.67}}} (0.10)& {\color{black}{\underline{2.10}}} (0.40)& {\color{black}{\textbf{1.55}}} (0.02)& {\color{black}{\textbf{1.55}}} (0.03)& {\color{black}{\textbf{1.73}}} (0.09)& {\color{black}{\textbf{1.59}}} (0.02)\\
 & 5& {\color{black}{\textbf{2.19}}} (0.14)& 2.28 (0.10)& {\color{black}{\underline{2.72}}} (0.30)& {\color{black}{\textbf{2.20}}} (0.07)& {\color{black}{\textbf{2.14}}} (0.20)& 2.39 (0.19)& {\color{black}{\textbf{2.19}}} (0.06)\\
 & 10& 3.42 (0.09)& 3.38 (0.05)& {\color{black}{\underline{4.01}}} (0.10)& 3.46 (0.27)& 3.56 (0.22)& 3.90 (0.22)& 3.72 (0.18)\\\hline
 & 2& {\color{black}{\textbf{0.29}}} (0.08)& 0.43 (0.06)& {\color{black}{\textbf{0.30}}} (0.08)& {\color{black}{\textbf{0.36}}} (0.06)& {\color{black}{\textbf{0.30}}} (0.04)& {\color{black}{\textbf{0.38}}} (0.07)& {\color{black}{\textbf{0.40}}} (0.06)\\
 WFG2& 3& {\color{black}{\textbf{0.62}}} (0.08)& 0.78 (0.07)& {\color{black}{\underline{0.82}}} (0.06)& 0.67 (0.08)& {\color{black}\mymk{\textbf{0.54}}} (0.07)& 0.75 (0.08)& 0.67 (0.08)\\
 & 5& {\color{black}{\textbf{1.34}}} (0.45)& 1.71 (0.21)& {\color{black}{\underline{1.80}}} (0.24)& {\color{black}{\textbf{1.40}}} (0.27)& {\color{black}{\textbf{1.39}}} (0.42)& {\color{black}{\textbf{1.65}}} (0.27)& {\color{black}{\textbf{1.41}}} (0.45)\\
 & 10& {\color{black}{\textbf{3.36}}} (0.86)& 4.29 (0.47)& {\color{black}{\underline{4.34}}} (0.44)& {\color{black}{\textbf{4.19}}} (0.27)& 4.25 (0.57)& {\color{black}{\textbf{4.18}}} (0.64)& 4.32 (0.45)\\\hline
 & 2& 0.35 (0.03)& 0.44 (0.03)& {\color{black}\mymk{\textbf{0.15}}} (0.05)& 0.37 (0.04)& 0.23 (0.03)& 0.31 (0.03)& 0.24 (0.03)\\
 WFG3& 3& 0.40 (0.04)& {\color{black}{\underline{0.56}}} (0.03)& {\color{black}\mymk{\textbf{0.27}}} (0.09)& 0.46 (0.05)& 0.39 (0.05)& {\color{black}{\textbf{0.34}}} (0.05)& 0.37 (0.06)\\
 & 5& {\color{black}{\textbf{0.35}}} (0.06)& 0.66 (0.06)& 0.52 (0.18)& 0.63 (0.04)& {\color{black}{\textbf{0.42}}} (0.06)& {\color{black}{\textbf{0.38}}} (0.06)& {\color{black}\mymk{\textbf{0.34}}} (0.06)\\
 & 10& {\color{black}\mymk{\textbf{0.79}}} (0.09)& 1.05 (0.08)& 1.10 (0.11)& 1.05 (0.13)& 0.97 (0.11)& {\color{black}{\textbf{0.85}}} (0.05)& {\color{black}{\textbf{0.86}}} (0.11)\\\hline
 & 2& {\color{black}\mymk{\textbf{0.19}}} (0.03)& 0.32 (0.09)& {\color{black}{\textbf{0.26}}} (0.13)& 0.31 (0.02)& {\color{black}{\textbf{0.28}}} (0.07)& 0.34 (0.12)& 0.35 (0.10)\\
 WFG4& 3& {\color{black}{\textbf{0.46}}} (0.06)& 0.67 (0.10)& 0.68 (0.25)& 0.68 (0.08)& 0.70 (0.13)& {\color{black}{\underline{0.87}}} (0.20)& {\color{black}\mymk{\textbf{0.45}}} (0.06)\\
 & 5& {\color{black}{\textbf{1.52}}} (0.16)& 2.39 (0.19)& {\color{black}{\underline{3.00}}} (0.30)& 2.50 (0.37)& 2.72 (0.42)& 2.82 (0.25)& {\color{black}{\textbf{1.59}}} (0.17)\\
 & 10& 9.84 (0.64)& 10.37 (0.27)& {\color{black}{\underline{11.89}}} (0.34)& 11.67 (0.54)& 11.84 (0.34)& 8.00 (0.47)& 9.71 (0.46)\\\hline
 & 2& 0.32 (0.03)& 0.48 (0.05)& {\color{black}\mymk{\textbf{0.20}}} (0.06)& {\color{black}{\textbf{0.26}}} (0.06)& 0.34 (0.05)& 0.47 (0.07)& 0.44 (0.08)\\
 WFG5& 3& {\color{black}\mymk{\textbf{0.59}}} (0.03)& 0.81 (0.06)& {\color{black}{\textbf{0.64}}} (0.15)& {\color{black}{\textbf{0.72}}} (0.12)& {\color{black}{\textbf{0.61}}} (0.07)& 0.73 (0.07)& {\color{black}{\textbf{0.62}}} (0.08)\\
 & 5& {\color{black}{\textbf{1.98}}} (0.23)& 2.30 (0.14)& {\color{black}{\underline{2.53}}} (0.15)& 2.07 (0.10)& {\color{black}{\textbf{2.03}}} (0.15)& 2.25 (0.15)& {\color{black}\mymk{\textbf{1.79}}} (0.10)\\
 & 10& 9.36 (0.26)& 9.12 (0.27)& {\color{black}{\underline{9.43}}} (0.27)& 9.39 (0.28)& {\color{black}\mymk{\textbf{8.37}}} (0.46)& 9.32 (0.25)& 9.14 (0.26)\\\hline
 & 2& {\color{black}{\textbf{0.29}}} (0.05)& 0.42 (0.04)& {\color{black}\mymk{\textbf{0.25}}} (0.06)& 0.54 (0.04)& {\color{black}{\textbf{0.31}}} (0.06)& 0.38 (0.07)& 0.42 (0.07)\\
 WFG6& 3& {\color{black}{\textbf{0.57}}} (0.05)& 0.74 (0.05)& 0.68 (0.23)& {\color{black}{\underline{0.89}}} (0.08)& {\color{black}{\textbf{0.63}}} (0.07)& {\color{black}{\textbf{0.65}}} (0.11)& {\color{black}\mymk{\textbf{0.53}}} (0.05)\\
 & 5& {\color{black}\mymk{\textbf{1.41}}} (0.06)& 2.15 (0.10)& {\color{black}{\underline{2.26}}} (0.18)& 2.24 (0.15)& 2.16 (0.11)& 1.77 (0.19)& {\color{black}{\textbf{1.58}}} (0.09)\\
 & 10& 8.74 (0.29)& 8.88 (0.19)& 8.92 (0.17)& {\color{black}{\underline{8.93}}} (0.18)& 8.79 (0.21)& 8.83 (0.22)& 8.82 (0.21)\\\hline
 & 2& 0.30 (0.03)& 0.43 (0.05)& {\color{black}\mymk{\textbf{0.15}}} (0.05)& 0.34 (0.03)& 0.24 (0.03)& 0.32 (0.02)& 0.30 (0.04)\\
 WFG7& 3& 0.63 (0.04)& 0.77 (0.05)& {\color{black}\mymk{\textbf{0.48}}} (0.08)& 0.62 (0.02)& 0.76 (0.11)& 0.63 (0.06)& 0.59 (0.04)\\
 & 5& {\color{black}{\textbf{1.85}}} (0.18)& 2.36 (0.16)& 2.13 (0.21)& 2.16 (0.11)& 2.58 (0.18)& 2.40 (0.26)& {\color{black}\mymk{\textbf{1.74}}} (0.12)\\
 & 10& 10.17 (0.26)& {\color{black}\mymk{\textbf{9.34}}} (0.43)& 10.17 (0.42)& 10.14 (0.35)& 10.12 (0.26)& 10.16 (0.26)& {\color{black}{\textbf{9.91}}} (0.30)\\\hline
 & 2& {\color{black}{\textbf{0.67}}} (0.03)& {\color{black}{\textbf{0.65}}} (0.03)& {\color{black}{\textbf{0.66}}} (0.08)& {\color{black}{\textbf{0.66}}} (0.04)& {\color{black}{\textbf{0.69}}} (0.06)& {\color{black}{\textbf{0.69}}} (0.03)& {\color{black}{\textbf{0.69}}} (0.03)\\
 WFG8& 3& {\color{black}{\textbf{0.91}}} (0.03)& {\color{black}{\textbf{0.98}}} (0.02)& {\color{black}{\underline{1.14}}} (0.21)& {\color{black}{\textbf{0.93}}} (0.11)& 1.10 (0.13)& {\color{black}{\textbf{0.92}}} (0.03)& {\color{black}\mymk{\textbf{0.89}}} (0.03)\\
 & 5& {\color{black}{\textbf{2.07}}} (0.15)& {\color{black}{\textbf{2.18}}} (0.08)& {\color{black}{\underline{2.92}}} (0.15)& 2.66 (0.30)& 2.88 (0.15)& 2.64 (0.20)& {\color{black}\mymk{\textbf{1.96}}} (0.05)\\
 & 10& 10.07 (0.23)& {\color{black}\mymk{\textbf{8.32}}} (0.69)& {\color{black}{\underline{10.12}}} (0.24)& 10.01 (0.32)& 10.06 (0.22)& 10.09 (0.26)& 9.76 (0.36)\\\hline
 & 2& {\color{black}{\textbf{0.23}}} (0.07)& 0.49 (0.06)& {\color{black}\mymk{\textbf{0.12}}} (0.06)& 0.48 (0.07)& 0.38 (0.12)& 0.44 (0.11)& 0.41 (0.08)\\
 WFG9& 3& {\color{black}\mymk{\textbf{0.44}}} (0.10)& {\color{black}{\underline{0.92}}} (0.07)& 0.76 (0.24)& 0.71 (0.11)& {\color{black}{\textbf{0.60}}} (0.14)& 0.84 (0.10)& {\color{black}{\textbf{0.60}}} (0.11)\\
 & 5& {\color{black}\mymk{\textbf{1.81}}} (0.14)& 2.45 (0.15)& 2.40 (0.28)& 2.28 (0.11)& {\color{black}{\textbf{2.04}}} (0.16)& 2.24 (0.23)& {\color{black}{\textbf{1.86}}} (0.19)\\
 & 10& {\color{black}{\textbf{9.18}}} (0.24)& {\color{black}{\textbf{9.25}}} (0.24)& {\color{black}{\underline{9.31}}} (0.22)& {\color{black}{\textbf{9.21}}} (0.24)& {\color{black}{\textbf{9.26}}} (0.24)& {\color{black}{\textbf{9.19}}} (0.28)& {\color{black}{\textbf{9.17}}} (0.20)\\\hline
\end{tabular} 
\caption{\label{tab:IGD_WFG}, Mean IGD values and standard deviation (in parentheses) for WFG problems. The values statistically similar to the best one are in bold, the best value is encircled the worst value is underlined}
\end{table*}

==> Supplementary_material.tex <==
Supplementary material

\section{Supplementary material}

\subsection{Sensitivity of HypI towards reference point}

\subsection{Sensitivity of function towards the number of objectives}

\subsection{Approximated Pareto fronts}


% \input{HV_WFG_Table.tex}

==> table_scfs.tex <==
\begin{table*}[tbp]
\caption{Scalarizing functions, their merits and demerits considered in this work}
\label{tab:scalarizing_functions}
\centering
\begin{tabular}{|p{5cm}|p{5cm}||p{5cm}||}
\hline

\textbf{Scalarizing function} & \textbf{Advantages} &\textbf{Limitations} \\ \hline

%Weighted compromising (WCP) & & \\ \hline
Weighted sum (WS) & one of the simplest way to scalarize multiple objectives, solution of the scalarized problem is weakly Pareto optimal \cite{Miettinen1999} & not suitable for non-convex Pareto fronts\\ \hline
Exponential weighted criterion (EWC) & & \\ \hline
 Weighted power (WPO) & & \\ \hline
 Weighted power (WPR) & & \\ \hline
 Weighted norm (WN) & & \\ \hline
 Chebyshev function (TCH) & & loses diversity for more than three objectives \cite{Coello2015,Zhang2007}\\ \hline
 Augmented Chebyshev (ATCH) & & \\ \hline
 Modified Chebyshev (MTCH) & & \\ \hline
 Achievement scalarizing function (ASF) & & \\ \hline
 Augmented achievement scalarizing function (AASF) & & \\ \hline
 Penalty boundary intersection (PBI) & & performance depends on the parameter $\theta$\\ \hline
 Quadratic PBI \cite{Hisao2016} (it needs value of $\alpha$) & & \\ \hline
 Inverted penalty boundary intersection (IPBI) & & \\ \hline
 Conic scalarizing function (CS) & & \\ \hline
 Vector angle distance scaling (VADS) & & \\ \hline
 Angle penalized distance (APD) \cite{Ran2016} & & \\ \hline
 Multiplicative scalarizing function (MSF) \cite{Jiang2018} & & \\ \hline
 Penalty based scalarizing function (PSF) \cite{Jiang2018} & & \\ \hline
 Hypervolume improvement (HypI) \cite{Alma2017} & Pareto compliance & \begin{enumerate} \item not suitable for many-objectives as it uses Pareto dominance in finding the values of scalarized function, \item computationally expensive especially for many-objectives, \item setting a reference point \end{enumerate} \\ \hline
 Dominance ranking (DomRank) \cite{Alma2017} & & \\ \hline
 Minimum Signed Distance (MSD) \cite{Alma2017} & &  Highly multimodal \\ \hline
\end{tabular}
\end{table*}


